A Deep Learning Mechanism for Efficient Information Dissemination in Vehicular Floating Content

Handling the tremendous amount of network data, produced by the explosive growth of mobile traffic volume, is becoming of main priority to achieve desired performance targets efficiently. Opportunistic communication such as FloatingContent (FC), can be used to offload part of the cellular traffic volume to vehicular-to-vehicular communication (V2V), leaving the infrastructure the task of coordinating the communication. Existing FC dimensioning approaches have limitations, mainly due to unrealistic assumptions and on a coarse partitioning of users, which results in over-dimensioning. Shaping the opportunistic communication area is a crucial task to achieve desired application performance efficiently. In this work, we propose a solution for this open challenge. In particular, the broadcasting areas called Anchor Zone (AZ), are selected via a deep learning approach to minimize communication resources achieving desired message availability. No assumption required to fit the classifier in both synthetic and real mobility. A numerical study is made to validate the effectiveness and efficiency of the proposed method. The predicted AZ configuration can achieve an accuracy of 89.7%within 98% of confidence level. By cause of the learning approach, the method performs even better in real scenarios, saving up to 27% of resources compared to previous work analytically modelled

==> misc-old/intro_old.tex <==
\section{Introduction}

%%%%%% intro
New offloading techniques to cope with the explosive growth in mobile traffic volumes, %and for the use cases as well as quality of service (QoS), 
are a fundamental component of the next generation radio access network (5G). %In vehicular ad-hoc networks (VANETs), 
Part of the cellular traffic volume can be offloaded to vehicular-to-vehicular communications (V2V), leaving to the infrastructure the task of managing and coordinating the communication.
In this context, of special interest are communication paradigms such as Floating Content (FC), an opportunistic communication scheme for the local dissemination of information \cite{floating}.  %\gr{small intro of FC. Done!}.

 FC beeing an infrastructure-less communication model, enables probabilistic contents storing in geographically constrained locations - denoted as \textit{Anchor Zones} (AZ) - and over a limited amount of time (i.e., application-based).
 
Since FC has been introduced, studies have focused mainly on its modeling, try to adjust it into a variant of scenarios from the Internet of Things (IoT)~\cite{office} to the Vehicular Ad-hoc Network (VANET)~\cite{itc29}. In particular, FC is based on the AZ area, where the opportunistic content exchange between nodes takes place (e.g., pedestrians, vehicles or hybrid communication) making the content "floats" without infrastructure needs. Only recently in~\cite{ours2017mobiworld}, a particular focus has fallen on Anchor Zone dimensioning. %%%%The gain respect to the other works
% However, in both paths, FC modeling and AZ reshaping, previous studies did not take into account the following main features: 
% \begin{itemize}
%   \item nodes mobility update on content received (i.e., event-based mobility),
%   \item anchor zone granularity in terms of road-grid which reduces the area not interest to the communication,
%   \item and, most notably, the high dynamic of nodes mobility which requires a time-based approach. 
% \end{itemize}
% This work adds to the FC state-of-the-art the above keys points. 
Existing approaches for FC dimensioning present the following issues:
\begin{itemize}
\item They are based on a coarse partitioning of users, which results in over dimensioning;
\item They are based on stationary assumption. In practical settings this applies to contents which are relatively long lived (a few hours, and in contexts in which mobility patterns and features do not vary significantly during content lifetime. Otherwise, a conservative approach is required again, based on the worst mobility conditions (in terms of node densities and contact rate) during the considered time interval. And this brings to severely overdimensioning of the AZ and to heavily overestimating the required amount of resources for achieving a specific performance goal.
\item The stationary analysis is completely useless for very short lived contents (less than one hour), as it does not accounts for the transient and the dynamics of content diffusion.  
\item The stationary analysis does not address the issue of optimal content seeding. In limit cases, the content must be seeded very frequently, thus defeating the purpose of FC as a mean of offloading cellular infrastructure.
\item Existing approaches are also based on the implicit assumption that mobility is not affected by information spreading. However, in most scenarios of interest, this is not the case. In a disaster scenario, for instance, floating the information about where rescue is needed, or where resources are available/unavailable, or where are hazards, clearly changes mobility patterns in ways that affect FC performance in return. Similar issues are found in swarms of drones for find and rescue operations, and even in pedestrian mobility, for messages about commercial sales, about flash events, about terrorist attacks, just to name a few. In these applications, how to  adequately engineer the FC paradigm without jeopardizing the communication resources available locally, achieving a target application performance while minimizing resource usage (in terms of bandwidth and/or memory, depending on the specific context), is an open issue which stands in the way of a practical deployment of the FC paradigm in such scenarios.
\end{itemize}
%
%%%Finally what we do!!!
%This study attempts to extend machine learning theory into floating content paradigm to tackle the traffic congestion issue.  
In this work, a machine learning (ML) approach has been used to adapt in real time FC parameters, in a way which achieves the target performance while minimizing the overall cost (modeled through a given cost function) during the whole duration of the congestion period. The model does not require any stationary assumption nor any geographical roadway-map information. Moreover, we believe that a massive data volume, variety features selection, and a tremendous number of dependency, can be analyzed only via an ML-based approach.
Therefore, a Convolutional Neural Network (CNN) over more ML techniques, has been used to predict the AZ configuration achieving an accuracy of $89.7\%$ within a confidence rate of $95\%$. Moreover, the predicted AZ configurations provide minor costs over the state-of-the-art results.   

Section~\ref{system_m} provides the system model assumption and measurements followed by Section~\ref{prob_f} which shows the notation used and the faced problem. CNN structure is shown in Section~\ref{alg} whereas Section~\ref{N-e} performs the numerical evaluations. Finally, in Section~\ref{related_w} we provide the related work, whereas, Section~\ref{concl} concludes this work.   


==> old.tex <==
\section{Problem Statement 2: circular AZ resizing subject to success ratio target (old try)}
\textbf{General goal:}  
The problem to save resources (such as bandwidth, spectrum, memory storage, energy) by using Floating Content approach in vehicular context. 

\textbf{State of the art:}
Previous works on FC focused mainly on the study of the probability of content floating, availability, and success probability performances. 


\textbf{Specific goal:}
In spite of FC constraints geographically information-spreading,
\textit{how to optimize resources used by FC over AZ size and shape is still an open challenge}. 

Our primary goal is to save resources reserving a certain level of FC performance. This can be done in several ways. For instance, without using an opportunistic replication but selecting which node is allowed to receive the content and which is not. Another approach, to efficiently save resources, is to choose a different shape than circular for the AZ (e.g., rectangular for a highway).   

In this work, we face the problem of circular anchor zone resizing (i.e., select the best radius) in order to reduce the amount of nodes involved in the communication preserving the target performances.  

\textbf{System model:}
We consider a $\mathbb{R}^2$ space where nodes move according to an arbitrary distribution. Assuming a stationary state, we suppose to know the mean moving time $T_m$, respectively the mean static time $T_s$ of the nodes.
We assume that nodes transmission range $r$ is the same for all the nodes (which can be extended for an arbitrary distribution). By contact, we refer to Gilbert's model. It means that a contact event happens when the distance between two nodes is less than $r$. We place a circular AZ with radius $R$, and we indicate the mean node sojourn time within AZ  as $T_{soj}$, the mean speed nodes as $v$, and the mean arrival rate as $\lambda$. 


\textbf{Approach:}
We consider a basic setting of FC with a circular AZ placed in XY. Following, \textit{we estimate, through a machine learning approach, the minimum AZ radius subject to some performance parameters} (e.g., target success rate) and applications requirements (e.g., a minimum, a maximum or both AZ size).   

\textbf{Main differences from our previous work:}
 Our earlier work, it is model based. This means that each gear, in the general process %shown in Fig.~\ref{fig:machine}
 , is given by the model took into account. However, in this work, we tackle the same issue without considering any model, and we want that the data give these gears. This is a machine learning problem.
 Moreover, in this work, we do not consider the homogeneity node density within AZ as in the previous work (i.e., we do not assume that nodes are uniformed distributed within AZ).
% \begin{figure}[h]
%  \begin{center}
%     \includegraphics[width=\columnwidth]{Presentation1.pdf}
% \caption{General process}
% \label{fig:machine}
% \end{center}
% \end{figure}

\textbf{Features:}
As a first attempt, we take into account $T_s$, $T_m$, $T_{soj}$, $\lambda$, $v$, $r$, $R$ as features. Moreover, we must consider application requirement such as minimum and maximum radius (resp. $R_{min}$, $R_{max}$). 


\textbf{Output:}
The output of our machine learning algorithm is $R$.
%which respect the application performances such as $R_{min}$, $R_{max}$, and target success probability $P_{succ}$


\textbf{Training set:}
The training set contains all the features previous mentioned. The larger, the better particularly using a deep learning technique. The training set vector values must be normalized in order to avoid local optimization. The \textit{p-norm} is the most suitable normalization for the types of features chosen. 


\textbf{Which learning is it:} 
The output of the machine is the value of $R \in \mathbb{R}$ which respect all the requirements. This is regression problem. 

\textbf{Machine learning technique}
Deep Boltzmann machine \textbf{(explain why or other option)}

\gr{Fundamental issue: Mobihoc again solves optimally this problem, and by not limiting shapes to circular, does better on average, than whatever you propose. there's no fundamental reason why you should limit AZ shape to circular.}




==> statement.tex <==
\section{Problem Statement 1: Floating Content Strategy to Avoid Traffic Congestion Using Machine Learning Theory}

%\gr{try again to define the problem you want to solve, in a way that does not leave room for interpretation.}


The fundamental idea is to use Floating Content to solve traffic congestion problem, by \textit{spreading the information concerning this issue, in the areas nearby the congestion zone}. We want to place the anchor zone (AZ), to inform other vehicles \textbf{to avoid} traffic hot-spots (congestion areas). To this end,  we need first to detect high-density vehicular areas then place the AZ in the most efficient zone (i.e., efficient in terms of resource usage and success ratio within the interest area).\\
%\gr{Unintelligible. what is the problem? what do you want to achieve?}\\

The problem can be split into two sub-problems: the \textit{traffic congestion detection (TCD)}, \textit{identification of the congestion zone}, that can be reused from the state of the art or by an ad-hoc algorithm,
%\gr{define accurately TC, and define TCD. What do you want to do? detect congestion? avoid congestion??}\\
and \textit{anchor zone positioning} in order to prevent other vehicles to enter the congestion area, where the core of our work is.\\

Placing a grid over a given map, where nodes move according to an arbitrary mobility model, we define $C_{congest}$ as the set of cells congested. $C_{congest}$ for instance, can be evaluated considering a mean speed threshold, below which the cells are congested. $C_{interest}$ is the set of cells interested to spread and store the content in order to inform all the nodes close to $C_{congest}$. Summarizing, $C_{congest}$ defines the congestion zones whereas, $C_{interest}$ defines the Anchor Zone. Finally, the aim of this work is to evaluate the minimum $C_{interest}$, given $C_{congest}$, and a success ratio target.   


As the first attempt, we assume that we do not change nodes mobility but only report the congestion issue. 





To face this issue, we use machine learning theory. So, without any analytical model to describe our scenario, we train the machine to extract the best area to place the AZ. Therefore, placing a grid on the whole region, via machine learning method we select which cells activate for content exchanging and storage. 

The training set features, machine learning techniques, and optimization part are still a work in progress. State of the art must be explored in deep. \\

\gr{No different than Mobihoc paper, which solves this issue optimally.}


















==> statement3.tex <==
\section{Problem Statement 3: A Floating Content Distributed Seeding Approach for Car Crash Situation}
To the best of our knowledge, previous works on floating content did not focus on seeding strategies. This open challenge, involve effects such as content sink and information spreading transitory which strongly influence any model performance outcomes.      
We consider a city map, where nodes move according an arbitrary distribution. At a specific time, a car crash occurred. A percentage of vehicles, surrounded the emergency zone have been selected as seeders (nodes that generate the message). The aim of this work, is to obtain the minimum seeding area subject to a success probability target measured over the board of a fixed AZ. Figure \ref{fig:seed_area} shows the crash location (in red), the seeding area (in blue), and the Anchor Zone (in black). 
\begin{figure}[h]
 \begin{center}
    \includegraphics[width=0.5\columnwidth]{seed_area.PNG}
\caption{Anchor Zone, seeding area and crash location}
\label{fig:seed_area}
\end{center}
\end{figure}

\gr{Seeding optimization is a relatively marginal issue}




==> statement_4.tex <==
\section{Problem formulation 4}

Considering stationary conditions is ok only for relatively stable settings and long lived contents.
In settings where mobility changes rapidly, and for short lived contents (1H or less), modeling of spatio temporal content evolution
becomes important.\\
You can start from Karlsson paper, and apply mobihoc approach.
The optimization problem now is an optimization over temporal sequences of choices for the replication and storage variables. 
Solving this optimally is the challenge. And you do not need necessarily machine learning for this.

\section{Problem 5}

Find a problem for which ML and the alike are a very good choice.

\section{Problem 6}
Same as problem 4, with the additional complication of having traffic react and change patterns as a consequence of information diffusion. You need a reasonable model for how traffic reacts to information, and solve 4 OPTIMALLY.
This is the coolest problem of all, so far.


